Multiagent Rollout with Reshuffling for Warehouse Robots Path Planning

Efficiently solving path planning problems for a large number of robots is critical to the successful operation of modern warehouses. The existing approaches adopt classical shortest path algorithms to plan in environments whose cells are associated with both space and time in order to avoid collision between robots. In this work, we achieve the same goal by means of simulation in a smaller static environment. Built upon the new framework introduced in (Bertsekas, 2021a), we propose multiagent rollout with reshuffling algorithm, and apply it to address the warehouse robots path planning problem. The proposed scheme has a solid theoretical guarantee and exhibits consistent performance in our numerical studies. Moreover, it inherits from the generic rollout methods the ability to adapt to a changing environment by online replanning, which we demonstrate through examples where some robots malfunction.

==> intro.tex <==
 
% E-commerce and logistic needs
In the recent years, the trade of goods over the internet, commonly referred as \emph{e-commerce} has consistently increased its influence, quickly taking over physical commerce thanks to its convenience to the consumer and large variety of options available. Companies involved in this business model have experience a massive growth, but must also deal with a large number of challenges in order to offer their services.

% Fulfillment centers
Fulfillment centers are the most critical part of the logistical infrastructures, massive warehouses tasked with the storage and handling of a large number of goods at the same time. The efforts to automatize these centers must deal with the challenge of coordinating hundreds of robots to transport items inside the warehouse efficiently.

    % Literature
    
% Basic Pathfinding
As computers became widely available to researches in the second half of the past century, complex problems such as the Shortest Path Problem (SPP) were approached with considerable success. Algorithms such as Bellman-Ford (\cite{bellman_routing_1958}), Dijkstra (\cite{dijkstra_note_1959}) and A* (\cite{hart_formal_1968}) exploited different properties of the problem to minimize the computational cost of solving the SPP.

% Multiagent Pathfinding
However, these methods only tackle single agent problems, limiting the range of applications. More recent effort have build upon previous methods to tackle several agents, algorithms such as Cooperative A* (\cite{silver_cooperative_2005}), M* (\cite{wagner_m_2011}) and Conflict Based Search (\cite{sharon_conflict-based_2015}) offer different possibilites in the tradeoff between computational cost and optimality for `multiagent pathfinding' (MAPF).

% Lifelong delivery
These algorithms are still unsuitable to deal with the environment of a common warehouse, as they only deal with one-shot problems, where each agent only has to move from one position to another. For a real environment, a robot is expected to move continuously, picking and delivering items. Such issue has been addressed recently (\cite{ma_lifelong_2017}, \cite{li_lifelong_2021})...

% Reinforcement Learning Intro
In parallel, the development of Reinforcement Learning (RL) has brought a collection of tools and frameworks to deal with complex problems. The generality of the framework provided by RL has encouraged its application in many different fields...
\cite{bertsekas2019reinforcement}

% Multiagent RL
Recent efforts in the RL learning fields have focused on tackling problems where several agents are involved. These problems deal with a control space that increases exponentially with the number of agents, rendering many problems of interest unfeasible for even powerful computation centers.

% Rollout applied to multiagent RL
Among the approaches developed to deal with this issue, a considerable success has been achieved with the use of multiagent rollout (\cite{bertsekas2021rollout}). By dealing with one agent at a time, the control space is dramatically decreases... 

==> numerical.tex <==
The environment used is a $47\times115$ grid-world with layout similar to the one used in \cite{wurman2008coordinating}. The agents are to collaboratively deliver $1183$ boxes to their designated delivery point, see implementation details [ref].

The numerical results are based on running cooperative
A* and multiagent rollout for 200 episodes for each agent
count, where an episode is determined complete when
all of the boxes are successfully delivered. Moreover, an
Apple M1 processor was used for all simulations and was
performed on a single thread.
\subsection{Runtime and memory consumption}

\definecolor{color1}{rgb}{0, 0.4470, 0.7410}
\definecolor{color2}{rgb}{0.8500, 0.3250, 0.0980}
\definecolor{color3}{rgb}{0.4660, 0.6740, 0.1880}
\tikzset{plotline/.style={line width=0.9}}
\tikzset{plotline1/.style={plotline, color=color1, mark=square}}
\tikzset{plotline2/.style={plotline, color=color2, mark=*}}
\tikzset{plotline3/.style={plotline, color=color3, mark=triangle}}

\begin{figure}
    \centering
    \vspace{1.6mm}
    \begin{tikzpicture}[trim axis left, trim axis right]
    \begin{axis}[
        xlabel={Number of agents $m$},
        ylabel={Success rate},
        xmin=100, xmax=200,
        ymin=0.5, ymax=1,
        width=7.5cm,
        height=4cm,
        xtick={100,150,200},
        ytick={},
        legend pos=south west,
        ymajorgrids=true,
        grid style=dashed,
        legend style={nodes={scale=0.6, transform shape}},
    ]
    
    \addplot[
        plotline1,
        ]
        coordinates {
        (100, 0.89)(110,0.9)(120,0.89)(130,0.84)(140,0.80)(150,0.79)(160, 0.72)(170, 0.76)(180, 0.67)(190, 0.67)(200, 0.58)
        };
    \addlegendentry{CA*}
    
    \addplot[
        plotline2,
        ]
        coordinates {
        (100, 1)(110,1)(120,1)(130,1)(140,1)(150,1)(160, 1)(170, 1)(180, 1)(190, 1)(200, 1)
        };
    \addlegendentry{MA-rollout}
        
        
    \end{axis}
    \end{tikzpicture}
        \caption{The average rate at which the methods are able to produce a feasible path.}
        \vspace{2mm}
        \label{fig:success_rate}
\end{figure}

\begin{figure}
    \centering

    \begin{tikzpicture}[trim axis left, trim axis right]
    \begin{axis}[
        xlabel={Number of agents $m$},
        ylabel={Runtime [ms]},
        xmin=100, xmax=200,
        ymin=5, ymax=60,
        width=7.5cm,
        height=4cm,
        xtick={100,150,200},
        ytick={10, 20, 30, 40, 50},
        legend pos=north west,
        ymajorgrids=true,
        grid style=dashed,
        legend style={nodes={scale=0.65, transform shape}},
    ]
    
    \addplot[
        plotline1,
        ]
        coordinates {
        (100, 19.0847)(110,20.6146)(120,22.2105)(130,24.2083)(140,25.9375)(150,27.9247)(160, 29.4)(170, 31.1875)(180, 32.5426)(190, 34.8866)(200, 38.5506)
        };
    \addlegendentry{CA*}
        
    \addplot[
        plotline2,
        ]
        coordinates {
        (100, 8.35895)(110,10.3783)(120,12.8847)(130,15.2359)(140,18.2616)(150,22.0642)(160, 25.5706)(170, 30.7799)(180, 35.61)(190, 42.7839)(200, 47.7844)
        };
    \addlegendentry{MA-rollout}
    
    \addplot[
        plotline3,
        ]
        coordinates {
        (100, 9.95)(110,11.93)(120,14.31)(130,16.7216)(140,20.5228)(150,24.1993)(160, 28.6255)(170, 33.6049)(180, 38.0182)(190, 45.5216)(200, 54.16)
        };
    \addlegendentry{MA-rollout w/o pre-comp.}
        
        
    \end{axis}
    \end{tikzpicture}
        \caption{The average time it takes to obtain  controls for all agents.}
        \label{fig:runtime}
\end{figure}

\begin{figure}
    \centering

    \begin{tikzpicture}[trim axis left, trim axis right]
    \begin{axis}[
        xlabel={Number of agents $m$},
        ylabel={$J_{\Tilde{\mu}}$},
        xmin=100, xmax=200,
        ymin=-15000000, ymax=-10000000,
        width=7.5cm,
        height=4cm,
        xtick={100,150,200},
        ytick={},
        legend pos=north east,
        ymajorgrids=true,
        grid style=dashed,
        legend style={nodes={scale=0.6, transform shape}},
    ]
    
    \addplot[
        plotline1,
        ]
        coordinates {
        (100, -11067000)(110,-11633200)(120,-12114500)(130,-12573800)(140,-12974900)(150,-13340400)(160, -13638800)(170, -13864100)(180, -14086000)(190, -14284500)(200, -14465500)
        };
    \addlegendentry{CA*}
    
    \addplot[
        plotline2,
        ]
        coordinates {
        (100, -10375300)(110,-10891900)(120,-11368100)(130,-11711800)(140,-11964700)(150,-12174700)(160, -12347200)(170, -12464300)(180, -12631600)(190, -12755200)(200, -12825800)
        };
    \addlegendentry{MA-rollout}
        
        
    \end{axis}
    \end{tikzpicture}
        \caption{The cumulative cost $J_{\Tilde{\mu}}$, averaged over 200 episodes. This is far smaller than $\Tilde{J}$, which has an average value of around $10^{20}$, verifying inequality \eqref{eq:cost_bound}.}
        \vspace{2mm}
        \label{fig:cumulative_reward}
\end{figure}

\begin{figure}
    \centering

    \begin{tikzpicture}[trim axis left, trim axis right]
    \begin{axis}[
        xlabel={Number of agents $m$},
        ylabel={Number of reshuffles},
        xmin=100, xmax=200,
        ymin=1, ymax=2.3,
        width=7.5cm,
        height=4cm,
        xtick={100,150,200},
        ytick={},
        legend pos=north east,
        ymajorgrids=true,
        grid style=dashed,
        legend style={nodes={scale=0.6, transform shape}},
    ]
    
    \addplot[
        plotline2,
        ]
        coordinates {
        (100, 1.2124)(110,1.23507)(120,1.27614)(130,1.3341)(140,1.3341)(150,1.48104)(160, 1.58021)(170, 1.62622)(180, 1.72564)(190, 1.90758)(200, 2.10627)
        };
        
        
    \end{axis}
    \end{tikzpicture}
        \caption{The average number of reshuffles needed. (MAYBE REMOVE?)}
        \vspace{2mm}
        \label{fig:number_of_shuffles}
\end{figure}


It is clear from Fig. \ref{fig:runtime} that Cooperative A* is slightly faster than multiagent rollout when there are more than 160 agents. However, one has to consider the lower success rate of Cooperative A* since only the successful computations runtime is part of the average. Furthermore, due to the parallel nature in which the approximations of the costs of each agent's controls are evaluated, one can imagine that it would be, in theory, possible to reduce the runtime of multiagent rollout by a factor of $C=5$ by doing these computations in parallel.


Additionally, the scale of the graph in which the shortest-path search is performed, differs between the methods. The graph needed by Cooperative A* is expected to be $N$ times larger than the graph used by the base policy of multiagent rollout, where $N$ denotes the time-steps needed for the agent to reach the target. This may therefore pose limitations on the maximum path-length of Cooperative A* from a memory standpoint.
\subsection{Adaptability}
Since the real-life operation of a warehouse is prone to unforeseen events, like robot malfunctioning, it is of great importance for a warehouse path-finding algorithm to be able to adapt to these circumstances. To investigate multiagent rollout's adaptability, we purposely simulated the total loss of control of some robots. More precisely, up to $20\%$ of robots were intentionally unable to move and the other agents regarded the grounded robots as having their base policy changed to one of complete stand-still. Remarkably, multiagent rollout adapted to this scenario, and the remaining agents continued their operation by circumnavigating these malfunctioned robots.

==> recycle.tex <==
In this section, we describe the multiagent rollout with random reshuffle algorithm, which is later applied to plan paths for warehouse robots. We will first introduce the multiagent optimal control problems with which we model the path planning problem of our interest, and then provide details of the rollout method. Our presentation is somewhat abstract, leaving further details specific to warehouse path planing to the next section.

\subsection{Multiagent Deterministic Optimal Control}
The problem considered here involves stationary dynamics
\begin{equation}
\label{eq:dynamics}
    x_{k+1}=f(x_k,u_k),\quad k=0,\,1,\,\dots,
\end{equation}
where $x_k$ and $u_k$ are state and control at stage $k$, which belong to state and control spaces $X$ and $U$, respectively, and $f$ maps $X\times U$ to $X$. Both the state and control spaces contain finitely many elements. The control $u_k$ must be chosen from a nonempty constraint set $U(x_k)\subset U$ that may depend on $x_k$. The multiagent nature of the problem manifests itself through the Cartesian product structure of $U(x_k)$, i.e.,
\begin{equation}
    \label{eq:cartesian}
    U(x_k)=U^1(x_k)\times \cdots \times U^m(x_k),
\end{equation}
where $m$ is an integer representing the number of agents involved in the problem. As a result, $u_k$ can be written as
$$u_k=(u_k^1,\dots,u_k^m),$$
with $u_k^i\in U^i(x_k)$, $i=1,\dots,m$. The cost of applying $u_k$ at state $x_k$ is denoted by $g(x_k,u_k)$, and is assumed to be real-valued.

We consider feedback policies of the form $\{\mu,\,\mu,\,\dots\}$, with $\mu$ being a function mapping $X$ to $U$ and satisfying $\mu(x)\in U(x)$ for all $x$. This type of polices are called \emph{stationary}. When no confusion arises, with a slight abuse of notation, we also denote $\{\mu,\,\mu,\,\dots\}$ as $\mu$. In view of the structure \eqref{eq:cartesian}, policy itself $\mu$ may be decomposed accordingly as
$$\mu(x)=\big(\mu^1(x),\dots,\mu^m(x)\big),$$
with $\mu^i(x)\in U_i(x)$, $i=1,\dots,m$. Accordingly, the system dynamics \eqref{eq:dynamics} and stage cost can be written as
$$x_{k+1}=f(x_k,u^1_k,\dots,u^m_k),\quad g(x_k,u^1_k,\dots,u^m_k)$$
respectively, with $u_k=(u^1_k,\dots,u^m_k)$ when stressing the multiagent structure of the problem.


The \emph{cost function} of a policy $\mu$, denoted by $J_\mu$, maps $X$ to the real line $\Re$, and is defined at any initial state $x_0 \in X$, as
\begin{equation}
\label{eq:pi_cost_function}
    J_\mu(x_0)= \sum_{k=0}^\infty \alpha^kg(x_k,\mu(x_k)),
\end{equation}
where $\alpha\in (0,1)$ is called \emph{discount factor}, which reflects the emphasis on the current cost over future ones, and $x_{k+1}=f(x_k,\mu(x_k))$, $k=0,\,1,\,\dots$. The limit in \eqref{eq:pi_cost_function} is well-posed in view of finiteness of $X$ and $U$. The optimal cost function $J^*$ is defined pointwise as
\begin{equation}
    J^*(x_0)=\inf_{u_k\in U(x_k),\ k=0,1,\ldots\atop x_{k+1}=f(x_k,u_k),\ k=0,1,\ldots}\sum_{k=0}^\infty  \alpha^kg(x_k,u_k).
\end{equation}
A stationary policy $\mu^*$ is called optimal if
\begin{equation*}
    J_{\mu^*}(x)=J^*(x),\quad \forall x\in X.
\end{equation*}

For the problem considered here, it can be shown that there exists a stationary optimal policy $\mu^*$; see, i.e., \cite[Props.~4.3.2 and 4.3.4]{bertsekas2019reinforcement}. Two exact DP algorithms for addressing the problem are value iteration (VI) and policy iteration (PI). However, these algorithms may be intractable, due to the \emph{curse of dimensionality}, which refers to the explosion of the computation as the cardinality of $X$ increases. Thus, various approximation schemes have been proposed, where one aims to obtain some suboptimal policy $\Tilde{\mu}$ such that $J_{\Tilde{\mu}}\approx J^*$. These schemes often involve minimizing some objective over the set $U(x)$. However, due to the structure \eqref{eq:cartesian} of $U(x)$, even those suboptimal scheme can be rather challenging as searching through the set $U(x)$ can be too costly as well. To see this, suppose each set $U^i(x)$ contains at most $N$ elements, then the total number of elements in $U(x)$ can be as large as $N^m$, which is prohibitively expensive to search through even for modest $m$. The multiagent rollout algorithm proposed in \cite{bertsekas2021multiagent} addresses exactly this problem, as we will discuss next.




The basis of our algorithm is that a function $\hat{J}:X\mapsto\Re$ that sets a realistic bound for the multiagent rollout policy is assumed to exist. We introduce permutation functions, denoted by $\sigma$ and $\tau$, which are one-to-one mappings with both domain and image being $\{1,\dots,m\}$. Thus, their inverse images exist and are denoted as $\sigma^{-1}$ and $\tau^{-1}$ respectively. 

Given the current state $x$ and permutation $\sigma$, we define $\tau_0=\sigma$. In addition, we define $\ell_0^i$ as
\begin{equation}
\label{eq:ell_tau}
    \ell_0^i=\tau_0^{-1}(i),\quad i=1,\dots,m.
\end{equation}
Then with a slight abuse of notation, we rearrange the elements of control according to $\tau_0$, i.e.,
$$u=\Big(u^{\ell_0^1},u^{\ell_0^2},\dots,u^{\ell_0^m}\Big),$$
and define control $\Tilde{u}_0$ via
\begin{equation}
    \label{eq:multi_rollout_tau}
        \begin{aligned}
    \Tilde{u}_0^{\ell_0^1}&\in\arg\min_{u^{\ell_0^1}\in U^{{\ell_0^1}}(x)}\Big\{g\big(x,u^{\ell_0^1},\mu^{\ell_0^2}(x),\dots,\mu^{\ell_0^m}(x)\big)\\
    &+\alpha J_\mu\Big(f\big(x,u^{\ell_0^1},\mu^{\ell_0^2}(x),\dots,\mu^{\ell_0^m}(x)\big)\Big)\Big\},\\
    \Tilde{u}_0^{\ell_0^2}&\in\arg\min_{u^{\ell_0^2}\in U^{{\ell_0^2}}(x)}\Big\{g\big(x,\Tilde{u}_0^{\ell_0^1},u^{\ell_0^2},\mu^{\ell_0^3}(x),\dots,\mu^{\ell_0^m}(x)\big)\\
    &+\alpha J_\mu\Big(f\big(x,\Tilde{u}_0^{\ell_0^1},u^{\ell_0^2},\mu^{\ell_0^3}(x),\dots,\mu^{\ell_0^m}(x)\big)\Big\},\\
    \dots& \qquad \dots\qquad \dots\\
    \Tilde{u}_0^{\ell_0^m}&\in\arg\min_{u^{\ell_0^m}\in U^{{\ell_0^m}}(x)}\Big\{g\big(x,\Tilde{u}_0^{\ell_0^1},\dots,\Tilde{u}_0^{\ell_0^{m-1}},u^{\ell_0^m}\big)\\
    &+\alpha J_\mu\Big(f\big(x,\Tilde{u}_0^{\ell_0^1},\dots,\Tilde{u}_0^{\ell_0^{m-1}},u^{\ell_0^m}\big)\Big)\Big\},
        \end{aligned}
\end{equation}
and define a control $\Tilde{u}_0$ as
$$\Tilde{u}_0=\Big(\Tilde{u}_0^{\ell_0^1},\Tilde{u}_0^{\ell_0^2},\dots,\Tilde{u}_0^{\ell_0^m}\Big).$$
In addition, a value $\hat{V}_0$ is defined similar to \eqref{eq:j_tilde} as
$$\hat{V}_0=g(x,\Tilde{u}_0)+\alpha J_\mu\big(f(x,\Tilde{u}_0)\big).$$

If $\hat{V}_0\leq \hat{J}(x)$, then we set $\Tilde{\mu}(x)=\Tilde{u}_0$. Otherwise, we generate according to certain probability distribution a new permutation $\tau_1$, define $\ell_1^i$ similar to \eqref{eq:ell_tau}, and carry out agent-by-agent optimization similar to \eqref{eq:multi_rollout_tau}. This procedure is repeated until after generating, say $j$, new permutations, the corresponding $\hat{V}_j$ fulfills that $\hat{V}_j\leq \hat{J}(x)$. Then we define $\Tilde{\mu}(x)=\Tilde{u}_j$, and the state $x'$ and permutation $\sigma'$ at the next stage is given by
$$x'=f\big(x,\Tilde{\mu}(x)\big),\quad \sigma'=\tau_j.$$

As stated earlier, the performance bound \eqref{eq:cost_bound} remains valid regardless of the order of agents being optimized. Thus, in view of the construction of $\Tilde{\mu}$, we have that 
$$J_{\Tilde{\mu}}(x)\leq \hat{J}(x),\quad \forall x\in X.$$


Efficiently solving path planning problems for a large number of robots is critical to the operation of modern warehouses. The existing approaches adopt classical shortest path algorithms to plan in environments whose cells are associated with both space and time in order to avoid collision between robots. In this work, we achieve the same goal by means of simulation in a smaller static environment. Built upon a new tool introduced in bertsekas, we propose a multiagent rollout with reshuffle algorithm, and apply it to address the problem of warehouse path planning. The proposed scheme has solid theoretical guarantees and exhibits consistent performance in our numerical studies. Moreover, it inherits the ability to adapt to a changing environment from the generic rollout methods, which we demonstrate through examples in which some robots malfunction. 
